Towards Zero-shot Language Modeling

Can we construct a neural model that is inductively biased towards learning human languages? Motivated by this question, we aim at constructing an informative prior over neural weights, in order to adapt quickly to held-out languages in the task of character-level language modeling. We infer this distribution from a sample of typologically diverse training languages via Laplace approximation. The use of such a prior outperforms baseline models with an uninformative prior (so-called "fine-tuning") in both zero-shot and few-shot settings. This shows that the prior is imbued with universal phonological knowledge. Moreover, we harness additional language-specific side information as distant supervision for held-out languages. Specifically, we condition language models on features from typological databases, by concatenating them to hidden states or generating weights with hyper-networks. These features appear beneficial in the few-shot setting, but not in the zero-shot setting. Since the paucity of digital texts affects the majority of the world's languages, we hope that these findings will help broaden the scope of applications for language technology.

==> aclrevision.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Created by Edoardo M. Ponti on 08/05/2020

% Disclaimer: there is no guarantee that the footer will appear as in ACL conference proceedings, as the commands below are reverse-engineered from the originals.

% Usage: Please follow these 2 steps:
% 1) Set the VARIABLES in the section below of the current file (up to "Do not modify anything beyond this point");
% 2) Insert the current file in your main LaTeX file by using \input{aclrevision} just before \begin{document}.

% Note: for 3-line footers, provide a value for \FirstLine; for 2-line footers, leave \FirstLine empty.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[pages=some]{background}
\usepackage{datetime}
\usepackage{etoolbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modify the following VARIABLES
\newcommand{\FirstPage}{2900}
\newcommand{\LastPage}{2910}
\newcommand{\Pages}[2]{\ifthenelse{\equal{#1}{#2}}{page #1}{pages #1--#2}}

% Leave \FirstLine empty for 2-line footers
\newcommand{\FirstLine}{Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing}
\newcommand{\SecondLine}{and the 9th International Joint Conference on Natural Language Processing,}
\newcommand{\ThirdLine}{Hong Kong, China, November 3--7, 2019. \textcopyright 2019 Association for Computational Linguistics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Do not modify anything beyond this point

\setcounter{page}{\FirstPage}
\thispagestyle{plain}
\pagestyle{plain}
\setlength\footskip{0.8cm}

\newcounter{Yloc}
\setcounter{Yloc}{15}

\newcommand{\citeinfo}[2]{
  \AddToShipoutPicture*{%
    \setlength{\unitlength}{1mm}
    \ifdefempty{\FirstLine}{}{
    \put(105,\value{Yloc}){\makebox(0,0){\footnotesize {\em \FirstLine}}} %
    \addtocounter{Yloc}{-4}
    }
    \put(105,\value{Yloc}){\makebox(0,0){\footnotesize {\em \SecondLine}~\Pages{\FirstPage}{\LastPage}}}
    \addtocounter{Yloc}{-4}
    \put(105,\value{Yloc}){\makebox(0,0){\footnotesize \ThirdLine}}
  }
}

\citeinfo{\FirstPage}{\LastPage}

\BgThispage
\SetBgColor{gray}
\SetBgContents{\huge ACL Anthology [revision] \the\day ~\shortmonthname[\the\month]~\the\year}% Set contents
\SetBgPosition{-0.9\marginparwidth,-0.5\textheight} % Select location
\SetBgOpacity{1.0}% Select opacity
\SetBgAngle{90.0}% Select rotation
\SetBgScale{1.}% Select scale factor
